A Tree-based Construction for Verifiable Diplomas with Issuer Transparency

Still to this day, academic credentials are primarily paper-based, and the process to verify the authenticity of such documents is costly, time-consuming, and prone to human error and fraud. Digitally signed documents facilitate a cost-effective verification process. However, vulnerability to fraud remains due to reliance on centralized authorities that lack full transparency. In this paper, we present the mechanisms we designed to create secure and machine-verifiable academic credentials. Our protocol models a diploma as an evolving set of immutable credentials. The credentials are built as a tree-based data structure with linked time-stamping, where portions of credentials are distributed over a set of smart contracts. Our design prevents fraud of diplomas and eases the detection of degree mills, while increasing the transparency and trust in the issuer's procedures. Our evaluation shows that our solution offers a certification system with strong cryptographic security and imposes a high level of transparency of the certification process. We achieve these benefits with acceptable costs compared to existing solutions that lack such transparency.

==> tex/contract-costs.tex <==
%!TEX root = ../main.tex

\makeatletter

\def\gas{36} % gwei
\def\ethusd{3344.20} % Exchange rate for ETH to USD
\def\daterate{2021-05-04} % Date of the exchange rate above

\def\@blockcertscred{21000 * \gas * \ethusd / 1e9}
\def\@issuecred{230641 * \gas * \ethusd / 1e9}
\def\@coursedeploy{3043997 * \gas * \ethusd / 1e9}
\def\@aggregation{114139 * \gas * \ethusd / 1e9}

\def\@blockcertscost#1{\@blockcertscred * #1}
\def\@examcost{\@issuecred}
\def\@coursecost#1{\@coursedeploy + #1 * \@examcost + \@aggregation}
\def\@semestercost#1#2{\@issuecred + #1 * (\@coursecost{#2})}
\def\@diplomacost#1#2#3{\@issuecred + #1 * (\@semestercost{#2}{#3}) + \@aggregation}

\def\@precision{\pgfkeys{/pgf/fpu,/pgf/number format/.cd,precision=2,/pgf/number format/fixed zerofill}}

\newcommand{\blockcertscost}[1]{%
\@precision\pgfmathparse{\@blockcertscost{#1}}\pgfmathprintnumber{\pgfmathresult}}

\newcommand{\examcost}{%
\@precision\pgfmathparse{\@examcost}\pgfmathprintnumber{\pgfmathresult}}

% Argument is number of exams
\newcommand{\coursecost}[1]{%
\@precision\pgfmathparse{\@coursecost{#1}}\pgfmathprintnumber{\pgfmathresult}}

% Argument 1: number of courses in semester
% Argument 2: number of exams per course
\newcommand{\semestercost}[2]{%
\@precision\pgfmathparse{\@semestercost{#1}{#2}}\pgfmathprintnumber{\pgfmathresult}}

% Argument 1: number semesters
% Argument 2: number of courses per semester
% Argument 3: number of exams per course
\newcommand{\diplomacost}[3]{%
\@precision\pgfmathparse{\@diplomacost{#1}{#2}{#3}}\pgfmathprintnumber{\pgfmathresult}}

\newcommand{\issuedcred}[1]{\pgfmathparse{#1}\pgfmathprintnumber{\pgfmathresult}}

\def\hashsize{32}
\def\addresssize{32}
\def\@credproofsize#1{(5 + #1) * \hashsize + (2 + #1) * \addresssize + 1}
\def\@credissuedsize#1{2 * \hashsize + \@credproofsize{#1}}
% Argument 1: number of credentials
% Argument 2: number of witnesses per credential (0 for leaf credentials)
\def\@credsize#1#2{\addresssize + #1 * \@credissuedsize{#2}}
% exam does not have witness
\def\@examcredsize{\@credsize{1}{0}}
\def\@coursecredsize#1{#1 * \@examcredsize}
\def\@semestercredsize#1#2{\@credsize{1}{#1} + #1 * (\@coursecredsize{#2})}
\def\@diplomacredsize#1#2#3{\@credsize{1}{#1} + #1 * (\@semestercredsize{#2}{#3})}

\def\inkbytes#1{(#1)/1000}

\newcommand{\blockcertssize}{\hashsize~b}

\newcommand{\blockcertsprogsize}[1]{%
\pgfmathparse{\inkbytes{#1 * \hashsize}}\pgfmathprintnumber{\pgfmathresult}~Kb}

\newcommand{\examcredsize}{%
\pgfmathparse{\@examcredsize}\pgfmathprintnumber{\pgfmathresult}~b}

% Argument 1: number of exams
\newcommand{\coursecredsize}[1]{%
\pgfmathparse{\@coursecredsize{#1}}\pgfmathprintnumber{\pgfmathresult}~b}

% Argument 1: number of courses per semester
% Argument 2: number of exams per course
\newcommand{\semestercredsize}[2]{%
\pgfmathparse{\inkbytes{\@semestercredsize{#1}{#2}}}\pgfmathprintnumber{\pgfmathresult}~Kb}

% Argument 1: number semesters
% Argument 2: number of courses per semester
% Argument 3: number of exams per course
\newcommand{\diplomacredsize}[3]{%
\pgfmathparse{\inkbytes{\@diplomacredsize{#1}{#2}{#3}}}\pgfmathprintnumber{\pgfmathresult}~Kb}

\makeatother

